Pretty Princess vs. Successful Leader: Gender Roles in Greeting Card Messages

People write personalized greeting cards on various occasions. While prior work has studied gender roles in greeting card messages, systematic analysis at scale and tools for raising the awareness of gender stereotyping remain under-investigated. To this end, we collect a large greeting card message corpus covering three different occasions (birthday, Valentine's Day and wedding) from three sources (exemplars from greeting message websites, real-life greetings from social media and language model generated ones). We uncover a wide range of gender stereotypes in this corpus via topic modeling, odds ratio and Word Embedding Association Test (WEAT). We further conduct a survey to understand people's perception of gender roles in messages from this corpus and if gender stereotyping is a concern. The results show that people want to be aware of gender roles in the messages, but remain unconcerned unless the perceived gender roles conflict with the recipient's true personality. In response, we developed GreetA, an interactive visualization and writing assistant tool to visualize fine-grained topics in greeting card messages drafted by the users and the associated gender perception scores, but without suggesting text changes as an intervention.

==> tables/GPT-2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[]
\begin{tabular}{l|l}
\hline
Prompt                                                                      & Following Message                                                                                                                                                                                                                                                 \\ \hline
Happy birthday sister!                                                      & \begin{tabular}[c]{@{}l@{}}Happy birthday sister! With many of you love your celebration! \\ It's time to celebrate with some cake and cake treats!\end{tabular}                                                                                                  \\ \hline
Happy birthday brother!                                                     & \begin{tabular}[c]{@{}l@{}}Happy birthday brother! You're on the cusp of a powerful \\  opportunity in life, and hopefully you and your family are enjoying it as much as\\ we are, making this magic happen.\end{tabular}                                          \\ \hline
Happy birthday dad!                                                         & \begin{tabular}[c]{@{}l@{}}Happy birthday dad! I hope you take care of this tool and make sure \\ it can move your family as comfortably as possible\end{tabular}                                                                                                 \\ \hline
Happy birthday mom!                                                         & \begin{tabular}[c]{@{}l@{}}Happy birthday mom! Woman, and girl! To the boy and girl who've \\ been in my life this year, thank you for having the patience to start \\ working in a non-obscene fashion at my house. You're old, know \\ your tricks\end{tabular} \\ \hline
Happy birthday grandfather!                                                 & \begin{tabular}[c]{@{}l@{}}Happy birthday grandfather! Thank you for making all my\\  life's history worth living. I hope to have much more fun\end{tabular}                                                                                                      \\ \hline
\begin{tabular}[c]{@{}l@{}}Happy birthday grandmother!\end{tabular} & \begin{tabular}[c]{@{}l@{}}Happy birthday grandmother! Looking forward to discovering \\ new bands and artists along the way! I think about things the way \\ they were meant to be shared…..\end{tabular}                                                  \\ \hline
\end{tabular}
\caption{Some sampled GPT-2 generated birthday greetings. }
\label{tab:gpt2}
\end{table}

==> tables/analysis_topics.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[]
% \begin{tabular}{l|l|l|l|l|l}
% \hline
%                   & dataset                   & age                                                     & female topics                                                                                                                                                                         & male topics                                                                                                                                                                            & gap  \\ \hline
% \multirow{8}{*}{B} & \multirow{4}{*}{template} & all                                                     & \begin{tabular}[c]{@{}l@{}}feminine, appearance, attractive, beauty, royalty, \\ fire, religion, anticipation,dispute, domestic work, \\ stealing, home, order, childish\end{tabular} & \begin{tabular}[c]{@{}l@{}}masculine, leader, work, philosophy, \\ social media, gain, competing, weather, \\ play, hearing, cold, achievement, ancient, \\ fun, business\end{tabular} & 3.50 \\ \cline{3-6} 
%                   &                           & babies                                                  & \begin{tabular}[c]{@{}l@{}}feminine, childish, affection, shape/size, \\ friends, love, surprise\end{tabular}                                                                         & \begin{tabular}[c]{@{}l@{}}achievenment, home, cold, ancient, violence, \\ divine, leisure\end{tabular}                                                                                & 1.46 \\ \cline{3-6} 
%                   &                           & parents                                                 & \begin{tabular}[c]{@{}l@{}}feminine, appearance, domestic work, beauty, \\ confusion, attractive, traveling, joy\end{tabular}                                                         & \begin{tabular}[c]{@{}l@{}}masculine, ancient, heroic, business, fun, \\ leisure, trust, shape and size\end{tabular}                                                                   & 4.19 \\ \cline{3-6} 
%                   &                           & \begin{tabular}[c]{@{}l@{}}grand\\ parents\end{tabular} & love, affection, home, family, ancient                                                                                                                                                & healing, celebration, optimism, friends, rural                                                                                                                                         & 0.94 \\ \cline{2-6} 
%                   & \multirow{4}{*}{GPT2}     & all                                                     & \begin{tabular}[c]{@{}l@{}}feminine, attractive, appearance, childish, \\ white collar job, fashion, home, clothing, \\ medical emergency, art, hipster, joy, sympathy\end{tabular}   & \begin{tabular}[c]{@{}l@{}}masculine, leader, play, death, wedding, \\ driving, swearing terms, dispute, alcohol, \\ strength, sound, toy, timidity\end{tabular}                       & 3.13 \\ \cline{3-6} 
%                   &                           & babies                                                  & \begin{tabular}[c]{@{}l@{}}feminine, childish, royalty, ocean, magic, \\ beach, appearance, water, sailing, \\ attractive, legend, beauty, fire, swimming\end{tabular}                & \begin{tabular}[c]{@{}l@{}}play, pet, technology, animal, hipster, valuable, \\ order, worship, sound, death, horror, sports, \\ programming, torment\end{tabular}                     & 9.05 \\ \cline{3-6} 
%                   &                           & parents                                                 & \begin{tabular}[c]{@{}l@{}}domestic work, phone, dispute, home, family, \\ pride, appearance, feminine, heroic, children,\\  hearing, divine\end{tabular}                             & \begin{tabular}[c]{@{}l@{}}leader, tourism, weather, restaurant, art, toy, \\ programming, cooking, play, \\ politeness, journalism, eating, shopping\end{tabular}                     & 3.59 \\ \cline{3-6} 
%                   &                           & \begin{tabular}[c]{@{}l@{}}grand\\ parents\end{tabular} & \begin{tabular}[c]{@{}l@{}}occupation, domestic work, death, \\ white collar job, feminine, hygiene,\\ rural, children, pride, furniture, joy, family\end{tabular}                    & \begin{tabular}[c]{@{}l@{}}pet, masculine, warmth, eating, fun, air travel,\\ messaging, shape and size, suffering, \\ achievement, weather, traveling\end{tabular}                    & 1.34 \\ \hline
% \multirow{4}{*}{V} & template                  & all                                                     & \begin{tabular}[c]{@{}l@{}}feminine, attractive, beauty, affection, \\ friends,  giving, love, optimism\end{tabular}                                                                  & \begin{tabular}[c]{@{}l@{}}nervousness, cold, pain, youth, shape/size,\\ party, achievement, fun\end{tabular}                                                                          & 1.53 \\ \cline{2-6} 
%                   & \multirow{3}{*}{GPT2}     & general                                                 & \begin{tabular}[c]{@{}l@{}}wedding, family, children, pride, worship,\\ cheerfulness, feminine, white collar job\end{tabular}                                                         & \begin{tabular}[c]{@{}l@{}}leader, play, eating, cooking, restaurant, \\ animal, liquid, smell, alcohol\end{tabular}                                                                   & 2.98 \\ \cline{3-6} 
%                   &                           & parents                                                 & \begin{tabular}[c]{@{}l@{}}domestic work, furniture, family, home,\\ hipster, tourism, internet\end{tabular}                                                                          & \begin{tabular}[c]{@{}l@{}}fire, art, emotional, writing, real estate, joy\\ cooking\end{tabular}                                                                                      & 1.32 \\ \cline{3-6} 
%                   &                           & \begin{tabular}[c]{@{}l@{}}grand\\ parents\end{tabular} & \begin{tabular}[c]{@{}l@{}}occupation, domestic work, dance, messaging,\\ furniture, college\end{tabular}                                                                             & masculine, tourism, sports, arts, zest, healing                                                                                                                                        & 1.20 \\ \hline
% \multirow{4}{*}{W} & template                  & all                                                     & \begin{tabular}[c]{@{}l@{}}sadness, feminine, attractive, beauty, children,\\ contentment, friends, affection\end{tabular}                                                            & \begin{tabular}[c]{@{}l@{}}wedding, childish, celebration, positive emotion, \\ cheerfulness, divine, party\end{tabular}                                                               & 0.85 \\ \cline{2-6} 
%                   & \multirow{3}{*}{GPT2}     & all                                                     & \begin{tabular}[c]{@{}l@{}}feminine, fashion, childish, appearance, fabric,\\ hipster, hygiene, clothing\end{tabular}                                                                 & \begin{tabular}[c]{@{}l@{}}leader, play, wedding, valuable, computer, \\ nervousness, music, banking, lust\end{tabular}                                                                & 6.41 \\ \cline{3-6} 
%                   &                           & parents                                                 & \begin{tabular}[c]{@{}l@{}}domestic work, home, sports, music, pride, \\ social media, deception, musical\end{tabular}                                                                & \begin{tabular}[c]{@{}l@{}}leader, hipster, sexual, fashion, swearing terms,\\ clothing, dispute, school\end{tabular}                                                                  & 3.49 \\ \cline{3-6} 
%                   &                           & \begin{tabular}[c]{@{}l@{}}grand\\ parents\end{tabular} & \begin{tabular}[c]{@{}l@{}}occupation, domestic work, fabric, clothing, \\ medical emergency, warmth, feminine, \\ appearance\end{tabular}                                            & \begin{tabular}[c]{@{}l@{}}journalism, cold, music, sports, musical, \\ banking, meeting, worship\end{tabular}                                                                         & 1.17 \\ \hline
% \end{tabular}
% \caption{Full male/female topic lists. Full version of Table~\ref{table:topic_list}}
% \end{table}
